The static quark potential and scaling behavior of SU(3) l attice Yang-Mills theory

The potential between a static quark and antiquark in pure SU(3) Yang-Mills theory is evaluated non-perturbatively through computations on the lattice in the region from short to intermediate distances (0.05 fm < r < 0.8 fm). In the high energy regime the results are compared with the parameter-free prediction of perturbation theory obtained by solving the Renormalization Group equation at two and three loops. The choice of the renormalization scheme to define a running coupling turns out to be important for the accuracy of the perturbative prediction: by obtaining the running coupling through the force, perturbation theory is applicable up to alpha ~ 0.3, while from the static potential only up to alpha ~ 0.15. In the region where perturbation is supposed to be reliable, no large unexpected non-perturbative term is observed. In the second part of this work, universality and scaling behavior of different formulations of Yang-Mills theory on the lattice are discussed, in particular the Iwasaki and DBW2 actions. The deconfinement temperature T_c*r0 and the glueball masses (m_0++)*r0, (m_2++)*r0 are analyzed. Particular attention is dedicated to the violation of physical positivity which occur in these actions and the consequences in the extraction of physical quantities from Euclidean correlation functions.

==> figures/loop <==
#FIG 3.2
Landscape
Center
Metric
A4      
100.00
Single
-2
1200 2
2 2 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 5
	 2700 2700 7650 2700 7650 5400 2700 5400 2700 2700
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 5175 2700 5400 2475
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 5175 2700 5400 2925
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 7650 3600 7425 3825
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 7650 3600 7875 3825
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 2475 4275 2700 4500
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 2700 4500 2925 4275
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 4500 5175 4725 5400
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 4725 5400 4500 5625
4 0 0 50 0 0 24 0.0000 4 225 105 5040 5760 t\001
4 0 0 50 0 0 24 0.0000 4 165 120 7875 4140 r\001

